IMP: Iterative Matching and Pose Estimation with Adaptive Pooling

Previous methods solve feature matching and pose estimation using a two-stage process by first finding matches and then estimating the pose. As they ignore the geometric relationships between the two tasks, they focus on either improving the quality of matches or filtering potential outliers, leading to limited efficiency or accuracy. In contrast, we propose an iterative matching and pose estimation framework (IMP) leveraging the geometric connections between the two tasks: a few good matches are enough for a roughly accurate pose estimation; a roughly accurate pose can be used to guide the matching by providing geometric constraints. To this end, we implement a geometry-aware recurrent attention-based module which jointly outputs sparse matches and camera poses. Specifically, for each iteration, we first implicitly embed geometric information into the module via a pose-consistency loss, allowing it to predict geometry-aware matches progressively. Second, we introduce an \textbf{e}fficient IMP, called EIMP, to dynamically discard keypoints without potential matches, avoiding redundant updating and significantly reducing the quadratic time complexity of attention computation in transformers. Experiments on YFCC100m, Scannet, and Aachen Day-Night datasets demonstrate that the proposed method outperforms previous approaches in terms of accuracy and efficiency.

==> figs_tables/fig_running_time.tex <==
%\setlength{\tabcolsep}{1.4pt}
\begin{figure}[t]
	\begin{minipage}{0.25\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/running_time}
		\caption{\textbf{Running time}.}
		\label{fig:running_time}
	\end{minipage}%
	\begin{minipage}{0.25\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/running_iteration}
		\caption{\textbf{Ratio of early stop}.}
		\label{fig:running_iteration}
	\end{minipage}
\end{figure}

==> figs_tables/table_ablation_aachen.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|cc}
			\toprule
			\textit{Feature} & \textit{Matcher} & Day & Night \\
			& & \multicolumn{2}{|c}{$(0.25m,2^\circ) / (0.5m,5^\circ) / (5m,10^\circ)$}\\
			\midrule
			
			\multirow{6}{*}{SuperPoint~\cite{superpoint}} 
			& Ours & 89.4 / 95.4 / 99.0 & 86.7 / 93.9 / 100.0  \\
			& Ours (w/p) & 89.1 / 95.4 / 99.0 & \textbf{86.7} / \textbf{94.9} / \textbf{100.0}\\
			& Ours (ada) & 90.2 / 96.2 / 99.0 & 84.7 / 93.9 / 100.0 \\
			& Ours (ada w/p) & \textbf{90.0} / \textbf{96.5} / \textbf{99.2} & 84.7 / \textbf{94.9} / \textbf{100.0} \\
	
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Ablation study of visual localization.}}
	\label{tab:ablation_aachen}
\end{table}

==> figs_tables/table_ablation_aachen_eimp.tex <==
\setlength{\tabcolsep}{4.0pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|cc}
			\toprule
			\textit{Feature} & \textit{Matcher} & Day & Night \\
			& & \multicolumn{2}{c}{$(0.25m,2^\circ) / (0.5m,5^\circ) / (5m,10^\circ)$}\\
			\midrule
			\multirow{2}{*}{SuperPoint~\cite{superpoint}} & EIMP w/o P & 90.0 / 96.5 / 99.2 & 84.7 / 94.9 / 100.0 \\
			& EIMP w/ P & 89.7 / 96.1 / 99.0 & 83.7 / 93.9 / 100.0 \\
			\midrule
			\multirow{2}{*}{SuperPoint~\cite{superpoint}} & EIMP w/o P & 90.0 / 96.5 / 99.0 & 77.0 / 91.6 / 99.5 \\
			& EIMP w/ P & 89.7 / 96.1 / 99.0 & 76.4 / 91.1 / 99.5 \\
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Ablation study on large-scale localization.} We test the performance of EIMP with (w/) and without (w/o) performing relative pose estimation (P) between the query and reference images in the localization process on Aachen v1.0 and Aachen v1.1 datasets~\cite{aachen,aachenv112021}.}
	\label{tab:ablation_aachen}
\end{table}

==> figs_tables/table_ablation_yfcc100m_old.tex <==
\setlength{\tabcolsep}{3.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|ccc|c|c}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{3}{|c|}{AUC} & \multirow{2}{*}{M.S.} & \multirow{2}{*}{Prec.(\%)}\\
			& &  $@5^\circ$ & $@10^\circ$ & $20^\circ$ & & \\
			\midrule
			\multirow{6}{*}{SuperPoint~\cite{superpoint}} 
			& SuperGlue (ours) & 36.9 & 57.1 & 73.7 & 23.7 & 85.2 \\
			& IMP-base & 38.6 & 58.3 & 74.6 & 23.6 & 87.2 \\
			& IMP-base w/g  & 39.1 & 59.0 & 75.0 & 23.7 & 87.7 \\
			& IMP-full & 39.4 & 59.4 & 75.2 & 23.0  & 84.9  \\
			& EIMP-base + pooling & 34.8 & 55.2 & 72.4 & 21.5 & 86.4 \\
			& EIMP-base & 36.4 & 56.5 & 73.0  & 18.4 & 88.8 \\
			& EIMP-base w/g & 36.9 & 56.6 & 73.3  & 18.4 & 88.7 \\
			& EIMP-base w/g + w/i & 37.2 & 57.2 & 73.3  & 18.3 & 86.5 \\
			& EIMP-full & 37.9 & 57.9 & 73.8 & 18.4 & 85.0\\ 
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Ablation study on feature matching.}}
	\label{tab:ablation_yfcc}
\end{table}

==> figs_tables/table_fm_bench.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table*}
	\footnotesize
	%\small
	%\scriptsize
	\centering
		\begin{tabular}{ll|cc|cc|cc|cc}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{2}{|c|}{CPC} & \multicolumn{2}{|c|}{T\&T} & \multicolumn{2}{|c|}{TUM} & \multicolumn{2}{|c}{KITTI}\\
			%\hline
			& & \textit{\%Recall}  & \textit{\#Corrs(-m)} 
			& \textit{\%Recall}  & \textit{\#Corrs(-m)} 
			& \textit{\%Recall}  & \textit{\#Corrs(-m)} 
			& \textit{\%Recall}  & \textit{\#Corrs(-m)} \\
			\midrule
			\multirow{4}{*}{RootSIFT~\cite{sift}} 
			& NN+RT & 52.9 & 92 (123) & 82.1 & 208 (287)  & 61.9 & 365 (438) & 90.6 & 847 (928) \\
			& AdaLAM~\cite{adalam} & 59.1 & 146 (216) & 81.4 & 307 (460) & 60.8 & 573 (798) & 90.6 & 981 (1116) \\ 
			& OANet~\cite{oanet} & 58.6 & 119 (167) & 84.7 & 219 (306) & 62.3 & 396 (454)  & 89.0 & 773 (854) \\
			& CLNet~\cite{clnet} & 54.0 & 171 (123)   & 70.9 & 217 (299) & 47.2 & 432 (532) & 88.4 & 746 (821) \\
			& SuperGlue~\cite{superglue} & 61.1 & 218 (466) & 86.8 & 382 (767) &  65.9 & 655 (1037) & 91.0 & 1261 (1746)  \\
			%& SuperGlue*~\cite{superglue} & & & & & & & & \\
			& SGMNet~\cite{sgmnet} & 62.0 & 248 (524) & 85.9 & 397 (789) & 66.6 & 704 (1132) & 91.2 & 1097 (1506) \\
			& Ours & 60.8 & 269 (714) & 87.1 & 467 (1020) & 65.1 & 901 (1698) & 89.5 & 1246 (1754)\\
			
			\midrule
			\multirow{4}{*}{SuperPoint~\cite{superpoint}} 
			& MNN & 34.5 & 152 (421) & 72.8 & 287 (717) & 56.7 & 280 (420) & 88.6 & 848 (1490) \\
			& AdaLAM~\cite{adalam} & 60.8 & 244 (640) & 90.6 & 398 (1001) & 55.2 & 731 (2185) & 86.7 & 935 (2173) \\
			& OANet~\cite{oanet} & 62.9 & 186 (343) & 91.2 & 280 (477) & 61.4 & 332 (473) & 82.2 & 482 (736) \\
			& CLNet~\cite{clnet} & 55.8 & 202 (424)   & 81.2 & 291 (589)  & 17.1 & 474 (811) & 83.6 & 732 (1226) \\ 
			& SuperGlue~\cite{superglue} & 68.8 & 287 (719) & 92.9 & 414 (987) & 59.1 & 512 (1038) & 88.7 & 957 (1777) \\
			& SuperGlue*~\cite{superglue} & 76.7 & 302 (712) & 96.6 & 431 (985) &  59.0 & 121 (177) & 89.5 & 354 (526) \\
			& SGMNet~\cite{sgmnet}& 70.3 & 327 (829) & 93.2 & 450 (1098) & 65.8 & 666 (1315) & 86.3 & 954 (1851) \\
			& Ours & 74.7 & 386 (1148) & 95.4 & 526 (1436) & 63.7 & 926 (2284) & 88.6 & 1009 (2072) \\
			& Ours (w / p) & 77.0 & 389 (1149) & 95.7 & 531 (1443) & 63.7 & 926 (2256) & 89.6 & 1020 (2085)  \\
			
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Results on FM-Bench dataset~\cite{fmbench}.}}
	\label{tab:fmbench}
\end{table*}

==> figs_tables/table_fm_bench_usac.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table*}
	\footnotesize
	%\small
	%\scriptsize
	\centering
		\begin{tabular}{ll|cc|cc|cc|cc}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{2}{|c|}{CPC} & \multicolumn{2}{|c|}{T\&T} & \multicolumn{2}{|c|}{TUM} & \multicolumn{2}{|c}{KITTI}\\
			%\hline
			& & \textit{\%Recall}  & \textit{\#Corrs(-m)} 
			& \textit{\%Recall}  & \textit{\#Corrs(-m)} 
			& \textit{\%Recall}  & \textit{\#Corrs(-m)} 
			& \textit{\%Recall}  & \textit{\#Corrs(-m)} \\
			\midrule
			\multirow{4}{*}{RootSIFT~\cite{sift}} 
			& NN+RT & 52.9 & 92 (123) & 82.1 & 208 (287)  & 61.9 & 365 (438) & 90.6 & 847 (928) \\
			& AdaLAM~\cite{adalam} & 59.1 & 146 (216) & 81.4 & 307 (460) & 60.8 & 573 (798) & 90.6 & 981 (1116) \\ 
			& OANet~\cite{oanet} & 58.6 & 119 (167) & 84.7 & 219 (306) & 62.3 & 396 (454)  & 89.0 & 773 (854) \\
			& CLNet~\cite{clnet} & 54.0 & 171 (123)   & 70.9 & 217 (299) & 47.2 & 432 (532) & 88.4 & 746 (821) \\
			
			& SuperGlue~\cite{superglue} & 74.5 & 360 (660) & 89.7 & 584 (1032) &  76.0 & 1091 (1691) & 90.1 & 1486 (2020)  \\
			%& SuperGlue*~\cite{superglue} & & & & & & & & \\
			& SGMNet~\cite{sgmnet} & 73.0 & 400 (664) & 88.6 & 596 (947) & 74.9 & 1179 (1650) & 88.1 & 1265 (1670) \\
			& Ours + w/p & 72.8 & 386 (714) & 91.2 & 607 (1020) & 75.7 & 1134 (1698) & 89.5 & 1429 (1754)\\
			& Ours (ada) + w/p & 72.8 & 336 (531) & 90.1 & 540.5 (814) & 75.7 & 1025 (1425) & 90.2 & 1295 (1479) \\
			
			\midrule
			\multirow{4}{*}{SuperPoint~\cite{superpoint}} 
			& MNN & 34.5 & 152 (421) & 72.8 & 287 (717) & 56.7 & 280 (420) & 88.6 & 848 (1490) \\
			& AdaLAM~\cite{adalam} & 60.8 & 244 (640) & 90.6 & 398 (1001) & 55.2 & 731 (2185) & 86.7 & 935 (2173) \\
			& OANet~\cite{oanet} & 62.9 & 186 (343) & 91.2 & 280 (477) & 61.4 & 332 (473) & 82.2 & 482 (736) \\
			& CLNet~\cite{clnet} & 55.8 & 202 (424)   & 81.2 & 291 (589)  & 17.1 & 474 (811) & 83.6 & 732 (1226) \\ 
			& SuperGlue~\cite{superglue} & 74.1 & 360 (660) & 89.2 & 584 (1032) & 76.3 & 1091 (1691) & 90.4 & 1486 (2019) \\
			& SuperGlue*~\cite{superglue} &  85.6 & 580 (977) & 97.9 & 731 (1247) & 74.8 & 1174 (1896) & 85.2 & 1371 (1973) \\
			& SGMNet~\cite{sgmnet}&  81.0 & 589 (993) & 95.8 & 748 (1290) & 71.0 & 1272 (2060) & 83.2 & 1346 (2170) \\
			& Ours &  86.4 & 613 (1148) & 97.5 & 773 (1436) & 74.5 & 1294 (2284) & 85.1 & 1381 (2072) \\
			& Ours (w / p) & 84.6 & 618 (1149) & 97.0 & 779 (1443) & 74.3 & 1273 (2223) & 84.8 & 1394 (2088)\\
			& Ours (ada) w/p & 83.4 & 527 (891) & 97.2 & 682 (1160) & 75.0 & 958 (1508) & 84.9 & 1168 (1644) \\
			
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Results on FM-Bench dataset~\cite{fmbench}.}}
	\label{tab:fmbench}
\end{table*}

==> figs_tables/table_scannet.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|ccc|c|c}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{3}{|c|}{AUC} & \multirow{2}{*}{M.S.} & \multirow{2}{*}{Prec.(\%)}\\
			& &  $@5^\circ$ & $@10^\circ$ & $20^\circ$ & & \\
			\toprule
			\multirow{6}{*}{RootSIFT~\cite{sift}} & NN+RT~\cite{sift} & 9.1 & 19.8 & 32.7 & 2.3 & 28.8 \\
			& AdaLAM (4k)~\cite{adalam} & 8.2 & 18.6 & 31.0 & 3.1 & 47.6 \\
			& OANet~\cite{oanet} & 10.71 &  23.10 & 37.42 & 3.20 & 36.93 \\
			& CLNet~\cite{clnet} & 5.8 & 15.1 & 26.8 & 2.0 & 43.9 \\
			& LMCNet~\cite{lmcnet} & 8.5 & 19.3 & 32.4 & - & 47.0 \\ 
			%& SuperGlue*~\cite{superglue} & & & & &\\
			& SuperGlue~\cite{superglue} & 13.1 & 28.0 & 43.9 & 8.5 & 42.5 \\
			& SGMNet\cite{sgmnet} & 12.8 & 27.9 & 44.6 & 8.8 & 45.6  \\
			& Ours & 14.6 & 30.7 & 47.5 & 9.9 & 42.8 \\
			& Ours (w/p) & 15.4 & 31.2 & 47.8 & 10.1 & 42.6 \\
			& Ours (w/p) + stop & 15.6 & 30.9 & 47.4 & 5.8 & 42.0 \\
			& Ours (ada) & 14.5 & 30.9 & 47.3 & 7.7 & 45.8 \\
			& Ours (ada w/p) & 14.7 & 30.4 & 47.3 & 7.5 & 46.2 \\
			& Ours (ada w/p) + early & 15.0 & 30.5 & 46.8 & 5.3 & 42.3 \\
			& Ours (ada w/p) + early + un & 15.3 & 30.8 & 46.6 & & \\ 
			\midrule
			
			\multirow{6}{*}{SuperPoint~\cite{superpoint}} 
			%& MNN & 5.0 & 12.8 & 24.3 & 17.1 & 17.1\\
			%& SuperGlue*~\cite{superglue} & 15.4 & 31.9 & 49.3 & 16.8 & 47.9 \\
			%& SuperGlue~\cite{superglue} &  12.4 & 26.6  & 42.4 & 15.0 & 45.9  \\
			%& SGMNet~\cite{sgmnet} & 16.3 & 31.8 & 48.7 & 17.0 & 48.2 \\
			% results from SGMNet
			& MNN & 9.4 & 21.6 & 36.4 & 13.3 & 30.2\\
			& AdaLAM (2k)~\cite{adalam} &  6.7 & 15.8 & 27.4 & 13.2 & 44.2  \\
			& OANet~\cite{oanet} &  10.0 & 25.1 &  38.0 &  10.6 & 44.6 \\
			& CLNet~\cite{clnet} & 4.1 & 11.0 & 21.6 & 8.6 & 44.2\\
			& LMCNet~\cite{lmcnet} & 14.6 & 33.6 & 53.6 & - & 36.8\\
			& SuperGlue~\cite{superglue} &  14.0 & 29.5 & 46.1 & 15.8 & 44.2  \\
			& SuperGlue*~\cite{superglue} & 16.2 & 33.8 & 51.9 & 18.5 & 47.3 \\
			& SGMNet~\cite{sgmnet} & 15.4 & 32.1 & 48.3 & 17.0 & 48.0 \\
			
			& Ours & 16.6 & 32.4 & 48.7 & 17.0 & 45.9 \\
			& Ours (w/p) & 16.5 & 32.5 & 49.1 & 17.1 & 46.2 \\
			
			& Ours (w/p) + early & 15.6 & 30.9 & 47.4 & 5.8 & 42.0 \\
			& Ours (ada) & 14.7 & 30.6 & 47.2 & 7.9 & 45.4 \\
			& Ours (ada + w/p) & 14.7 & 30.4 & 47.3 & 7.5 & 46.2 \\
			& Ours (ada + w/p) + stop & 15.0 & 30.5 & 46.8 & 5.3 & 42.3 \\
			& Ours (ada + w/p) + stop + un & 15.3 & 30.8 & 46.6 & & \\
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Results on Scannet dataset~\cite{scannet}.}}
	\label{tab:scannet}
\end{table}

==> figs_tables/table_scannet_new.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|ccc|c|c}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{3}{|c|}{AUC} & \multirow{2}{*}{M.S.} & \multirow{2}{*}{Prec.(\%)}\\
			& &  $@5^\circ$ & $@10^\circ$ & $20^\circ$ & & \\
			\toprule
			\multirow{6}{*}{RootSIFT~\cite{sift}} & NN+RT~\cite{sift} & 9.3 & 20.6 & 33.7 & 2.3 & 28.2 \\
			& AdaLAM (4k)~\cite{adalam} & 8.24 & 18.57 & 31.01 & 3.10 & 47.59 \\
			& OANet~\cite{oanet} & 10.71 &  23.10 & 37.42 & 3.20 & 36.93 \\
			& CLNet~\cite{clnet} & 4.9 & 12.9 & 23.5 & 2.8 & 37.5 \\
			& LMCNet~\cite{lmcnet} & 8.5 & 19.3 & 32.4 & - & 47.0 \\ 
			%& SuperGlue*~\cite{superglue} & & & & &\\
			& SuperGlue~\cite{superglue} & 13.8 & 29.2 & 45.2 & 8.4 & 42.2 \\
			& SGMNet\cite{sgmnet} & 13.0 & 27.8 &  44.2 & 8.8 & 45.5 \\
			
			\midrule
			
			\multirow{6}{*}{SuperPoint~\cite{superpoint}} 
			%& MNN & 5.0 & 12.8 & 24.3 & 17.1 & 17.1\\
			%& SuperGlue*~\cite{superglue} & 15.4 & 31.9 & 49.3 & 16.8 & 47.9 \\
			%& SuperGlue~\cite{superglue} &  12.4 & 26.6  & 42.4 & 15.0 & 45.9  \\
			%& SGMNet~\cite{sgmnet} & 16.3 & 31.8 & 48.7 & 17.0 & 48.2 \\
			% results from SGMNet
			& MNN & 5.0 & 12.8 & 24.3 & 17.1 & 17.1\\
			& AdaLAM (2k)~\cite{adalam} &  6.7 & 15.8 & 27.4 & 13.2 & 44.2  \\
			& OANet~\cite{oanet} &  10.0 & 25.1 &  38.0 &  10.6 & 44.6 \\
			& CLNet~\cite{clnet} & 4.1 & 11.0 & 21.6 & 8.6 & 44.2\\
			& LMCNet~\cite{lmcnet} & 14.6 & 33.6 & 53.6 & - & 36.8\\
			& SuperGlue*~\cite{superglue} & 15.4 & 31.9 & 49.3 & 16.8 & 47.9 \\
			& SuperGlue~\cite{superglue} &  12.4 & 26.6  & 42.4 & 15.0 & 45.9  \\
			& SGMNet~\cite{sgmnet} & 16.3 & 31.8 & 48.7 & 17.0 & 48.2 \\
			
			%& MNN & 9.44 & 21.57 & 36.41 & 13.27 & 30.17 \\
			%& SuperGlue~\cite{superglue} & 13.95 & 29.48 & 46.07 & 15.82 & 44.18 \\
			%& SuperGlue*~\cite{superglue} & 16.19 & 33.82 &  51.86 & 18.50  & 47.32 \\
			%& SGMNet~\cite{sgmnet} & 15.40 & 32.06 & 48.32 & 16.97 & 48.01 \\
			
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Results on Scannet dataset~\cite{scannet}.}}
	\label{tab:scannet}
\end{table}

==> figs_tables/table_yfcc100m.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|ccc|c|c}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{3}{|c|}{AUC} & \multirow{2}{*}{M.S.} & \multirow{2}{*}{Prec.(\%)}\\
			& &  $@5^\circ$ & $@10^\circ$ & $20^\circ$ & & \\
			\midrule
			\multirow{6}{*}{RootSIFT~\cite{sift}}
			%& NN + RT & 49.07 & 58.76 & 68.58 & 8.23 & 29.79 \\
			%& AdaLAM (4k) & 57.78 & 68.01 & 77.38 & 7.92 & 83.15 \\
			%& OANet~\cite{oanet} & 58.00 & 67.80 & 77.46 & 5.84 & 81.80 \\
			%& SuperGlue*~\cite{superglue} & 59.25 & 70.38 & 80.44 & - & -\\
			%& SuperGlue~\cite{superglue} & 63.82 & 73.33 & 82.26 & 16.59 & 81.08\\
			%& SGMNet\cite{sgmnet} & 62.72 & 72.52 & 81.48 & 17.08 & 86.08 \\
			
			& NN-RT~\cite{sift} & 26.7 & 43.2 & 59.4 & 4.4 &  56.4 \\
			& AdaLAM (4k)~\cite{adalam}& 27.5 & 44.5  & 60.5 & 6.3 & 84.3   \\
			& OANet~\cite{oanet}~\cite{oanet} & 22.4 & 36.3 & 50.3 & 5.6 & 53.74 \\
			& CLNet~\cite{clnet} & 33.0 & 52.1 & 68.5 & 7.82 & 75.2 \\
			& LMCNet~\cite{lmcnet} & 35.8 & 55.6 & 72.2 & - & 86.9 \\
			& SuperGlue*~\cite{superglue} & 35.3 & 56.1 & 73.6 & - & -\\
			& SuperGlue~\cite{superglue} & 35.2 & 55.3 & 72.3 & 17.0 & 81.7\\
			& SGMNet\cite{sgmnet} & 35.1 & 54.8 & 71.5 & 17.0 & 86.1 \\
			& ClusterGNN~\cite{clustergnn} &  32.8 & 50.3  & 65.9 & & \\
			& Ours & 36.3 & 56.1 & 72.5 & 17.5 & 84.2 \\
			& Ours (w/p) & 36.7 & 56.4 & 72.8 & 18.0 & 83.8\\
			& Ours (w/p) + stop & 36.7 & 56.6 & 72.9 & 18.0 & 77.6 \\
			& Ours (ada) & 36.4 & 56.1 & 72.5 & 13.8 & 87.3 \\
			& Ours (ada w/p) & 36.9 & 56.9 & 72.8 & 13.7 & 87.8 \\
			& Ours (ada w/p) + stop & 36.9 & 56.7 & 72.9 & 13.7 & 79.8 \\
			& Ours (ada w/p) + stop + un & 36.8 & 56.3 & 72.8 & 13.7 & 79.8 \\
			
			\midrule
			
			\multirow{6}{*}{SuperPoint~\cite{superpoint}} 
			& MNN & 6.5 &  15.4 & 28.5 & 16.2 & 16.2 \\
			& AdaLAM (2k)~\cite{adalam} & 20.8 & 36.5 & 51.9 & 10.9 & 72.0 \\
			& OANet~\cite{oanet} & 19.2 & 34.5 &  50.3 &  9.4 & 62.1\\
			& CLNet~\cite{clnet} & 27.8 & 46.4 & 63.8 & 11.9 & 75.1\\
			& LMCNet~\cite{lmcnet} & 17.4 & 33.2 & 51.1 & - & 88.9 \\
			& SuperGlue*~\cite{superglue} & 37.9 & 58.0 & 74.3 & 21.7 & \textbf{88.5} \\
			& SuperGlue~\cite{superglue} & 33.2 & 53.5 & 70.8 & 19.7 & 78.7 \\
			& SGMNet~\cite{sgmnet} & 33.0 & 53.0 & 70.0 & 22.3 &  85.1 \\
			& ClusterGNN~\cite{clustergnn} &  35.3 & 56.1 & 73.6 & - & -\\
			
			& Ours & 38.6 & 58.3 & 74.6 & 23.6 & 87.2 \\
			& Ours (w/p) & \textbf{39.1} & \textbf{59.0} & \textbf{75.0} & \textbf{23.7} & 87.7 \\
			& Ours (w/p) + stop & 39.4 & 59.4 & 75.2 & 84.9 & 23.0 \\
			& Ours (ada) & 36.4 & 56.5 & 73.0 & 88.8 & 18.4 \\
			& Ours (ada w/p) & 36.9 & 56.6 & 73.3 & 88.7 & 18.4 \\
			& Ours (ada w/p) + stop & 37.2 & 57.2 & 73.3 & 86.5 & 18.3 \\
			& Ours (ada w/p) + stop + un & 37.9 & 57.9 & 73.8 & 85.0 & 18.4 \\ 
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Results on YFCC100M dataset~\cite{yfcc100m}.}}
	\label{tab:yfcc}
\end{table}

==> figs_tables/table_yfcc100m_new.tex <==
\setlength{\tabcolsep}{4.pt}

\begin{table}
	%\footnotesize
	%\small
	\scriptsize
	\centering
		\begin{tabular}{ll|ccc|c|c}
			\toprule
			\multirow{2}{*}{\textit{Feature}} & \multirow{2}{*}{\textit{Matcher}} & \multicolumn{3}{|c|}{AUC} & \multirow{2}{*}{M.S.} & \multirow{2}{*}{Prec.(\%)}\\
			& &  $@5^\circ$ & $@10^\circ$ & $20^\circ$ & & \\
			\midrule
			\multirow{6}{*}{RootSIFT~\cite{sift}}
			%& NN + RT & 49.07 & 58.76 & 68.58 & 8.23 & 29.79 \\
			%& AdaLAM (4k) & 57.78 & 68.01 & 77.38 & 7.92 & 83.15 \\
			%& OANet~\cite{oanet} & 58.00 & 67.80 & 77.46 & 5.84 & 81.80 \\
			%& SuperGlue*~\cite{superglue} & 59.25 & 70.38 & 80.44 & - & -\\
			%& SuperGlue~\cite{superglue} & 63.82 & 73.33 & 82.26 & 16.59 & 81.08\\
			%& SGMNet\cite{sgmnet} & 62.72 & 72.52 & 81.48 & 17.08 & 86.08 \\
			
			& NN-RT~\cite{sift} & 26.7 & 43.2 & 59.4 & 4.4 &  56.4 \\
			& AdaLAM (4k)~\cite{adalam}& 27.5 & 44.5  & 60.5 & 6.3 & 84.3   \\
			& OANet~\cite{oanet}~\cite{oanet} & 22.4 & 36.3 & 50.3 & 5.6 & 53.74 \\
			& CLNet~\cite{clnet} & 33.0 & 52.1 & 68.5 & 7.82 & 75.2 \\
			& LMCNet~\cite{lmcnet} & 35.8 & 55.6 & 72.2 & - & 86.9 \\
			& SuperGlue*~\cite{superglue} & 35.3 & 56.1 & 73.6 & - & -\\
			& SuperGlue~\cite{superglue} & 35.2 & 55.3 & 72.3 & 17.0 & 81.7\\
			& SGMNet\cite{sgmnet} & 35.1 & 54.8 & 71.5 & 17.0 & 86.1 \\
			& ClusterGNN~\cite{clustergnn} &  32.8 & 50.3  & 65.9 & & \\
			
			\midrule
			
			\multirow{6}{*}{SuperPoint~\cite{superpoint}} 
			& MNN & 6.5 &  15.4 & 28.5 & 16.2 & 16.2 \\
			& AdaLAM (2k)~\cite{adalam} & 20.8 & 36.5 & 51.9 & 10.9 & 72.0 \\
			& OANet~\cite{oanet} & 19.2 & 34.5 &  50.3 &  9.4 & 62.1\\
			& CLNet~\cite{clnet} & 27.8 & 46.4 & 63.8 & 11.9 & 75.1\\
			& LMCNet~\cite{lmcnet} & 17.4 & 33.2 & 51.1 & - & 88.9 \\
			& SuperGlue*~\cite{superglue} & 37.9 & 58.0 & 74.3 & 21.7 & 88.5 \\
			& SuperGlue~\cite{superglue} & 33.2 & 53.5 & 70.8 & 19.7 & 78.7 \\
			& SGMNet~\cite{sgmnet} & 33.0 & 53.0 & 70.0 & 22.3 &  85.1 \\
	
			\bottomrule			   
		\end{tabular}
	\caption{\textbf{Results on YFCC100M dataset~\cite{yfcc100m}.}}
	\label{tab:yfcc}
\end{table}

==> sections_camera_ready/Abstract-20221110.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
	%In this paper, we propose \textbf{i}terative \textbf{m}atching and \textbf{p}ose estimation, dubbed IMP, to build correspondences between keypoints extracted from two images and estimate the relative pose iteratively in contrast to previous methods, which first find matches and then recover the pose from predicted matches sequentially. Our motivation is based on the relationship of the two tasks: several good matches are enough for a roughly accurate pose estimation; a roughly accurate pose can be further used to guide the matching by providing geometric constraints. Specifically, in the feature matching process, we leverage the powerful transformers to enhance the discriminative ability of keypoints with geometric information embedded. In the pose estimation process, geometry-aware matches are used for pose prediction. Once we find a good pose, the iteration stops and the good pose is used to find more accurate matches. To mitigate the quadratic time complexity of transformers, we introduce an \textbf{e}fficient version called EIMP to adaptively discard keypoints without matches in the other image, avoiding updating useless keypoints and thus leading to sub-linear matching complexity. In the sampling, we utilize the uncertainty of predicted pose to dynamically adjust the number of keypoints to be preserved, making the system more accurate. Our experiments on relative pose estimation and large-scale localization tasks demonstrate that the proposed method outperforms previous approaches in terms of accuracy but with higher efficiency.
	
	Previous methods solve feature matching and pose estimation separately by first finding matches and then estimating the pose. As they ignore the geometric relationships between the two tasks, they focus on either improving the quality of matches or filtering potential outliers, leading to limited efficiency or accuracy. In contrast, we propose an \textbf{i}terative \textbf{m}atching and \textbf{p}ose estimation framework (IMP) leveraging the geometric connections between the two tasks: several good matches are enough for a roughly accurate pose estimation; a roughly accurate pose can be used to guide the matching by providing geometric constraints. We adopt a geometry-aware recurrent module with transformers to perform matching and pose estimation iteratvely. Specifically, in the matching process, we implicitly embed geometric information via transformers to enhance the discriminativeness of keypoints. In the pose estimation process, geometry-aware matches are used to estimate the pose, which is further used to find more accurate matches via geometric guidance. Moreover, we introduce an \textbf{e}fficient IMP (EIMP) to dynamically discard keypoints without potential matches, avoiding redundant updating in transformers and changing the quadratic complexity of matching to sub-linear. By combining the matching quality, attention scores, and the uncertainty of poses, our sampling strategy achieves high efficiency and preserves the accuracy. Experiments on YFCC100m, Scannet, and Aachen Day-Night datasets demonstrate that the proposed method outperforms previous approaches in terms of accuracy and efficiency.
	
\end{abstract}

==> sections_camera_ready/Experiments-20221110.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we first give implementation details in Sec.~\ref{sec:imp}. Then, we compare our method with previous state-of-the-art (SOTA) approaches on relative pose estimation and visual localization tasks in Sec.~\ref{sec:matching} and Sec.~\ref{sec:localization}, respectively. Next, we analyze the computational cost in Sec.~\ref{sec:running_time}. Finally, we conduct a full ablation study in Sec.~\ref{sec:ablation}. More implementation details and results can be found in the \textbf{supplementary material}.

\subsection{Implementation details}
\label{sec:imp}
We implement the network in PyTorch~\cite{pytorch} and train it on the MegaDepth dataset~\cite{megadepth} for 900k iterations in total with Adam optimizer~\cite{adam}, batch size of 16, initial learning rate of 1e-4, weight decay of 5e-4. The learning rate decays with ratio of 0.99996 after 200k iterations and is fixed when it reaches 1e-5. We use 1024 keypoints extracted by SuperPoint (SP)~\cite{superpoint} and RootSIFT~\cite{sift,rootsift2012} for training. As SuperGlue~\cite{superglue}, our network has 9 ($N_t$) self-cross attention blocks. $\alpha_{m}, \alpha_{p}$, $\alpha_{g}$, $\theta_m$, $\theta_P$ are set to 0.6, 0.2, 0.2, 0.2, and 1.5, respectively. Note that unlike SuperGlue which is first pre-trained on Oxford and Paris dataset~\cite{oxford2018} and then fine-tuned on Scannet~\cite{scannet} and MegaDepth~\cite{megadepth} datasets for indoor and outdoor models respectively, all our models are trained only on the MegaDepth dataset~\cite{megadepth} from scratch. \textbf{We will release the source code including the training part for reproduction}.

\subsection{Relative pose estimation}
\label{sec:matching}

\textbf{Datasets.} We first test our method on the public YFCC100m~\cite{yfcc100m} and Scannet~\cite{scannet} datasets to evaluate the performance on relative pose estimation. YFCC100m~\cite{yfcc100m} is a large-scale outdoor dataset consisting of images with large illumination and season changes and viewpoint variations.  Scannet~\cite{scannet} is an indoor dataset widely used for depth prediction~\cite{probdepth2022} and pose estimation~\cite{superglue,sgmnet}. As SuperGlue~\cite{superglue}, we use 1.5k and 2k pairs in Scannet and YFCC100m datasets for evaluation, respectively.

% On FM-Bench dataset, as SGMNet,  we report the recall on fundamental matrix estimation (\%Recall) and the mean number of correct matches (\#Corrs(-m)) after/before RANSAC. We adopt the RANSAC with normalized symmetric epipolar distance (SGD) for fundamental matrix estimation. A match with normalized SGD lower than 0.05 (used by the original paper~\cite{fmbench}) is deemed as correct. For each image, we detect up to 4k keypoints.

\input{figs_tables/table_yfcc100m_usac}

\textbf{Metrics.} Following previous methods~\cite{superglue,sgmnet,clustergnn}, we report the accurate cumulative error curve (AUC)~\cite{superglue} at error thresholds of $5^\circ$, $10^\circ$, and $20^\circ$.  The error is the maximum angular errors of rotations and normalized translations. We also report the mean matching score (M.S.) and mean precision (Prec.) of predicted matches. We detect 2k keypoints for both RootSIFT~\cite{sift,rootsift2012} and SuperPoint~\cite{superpoint} keypoints on YFCC100m dataset, while on Scannet dataset, we detect 2k keypoints for RootSIFT and 1k for SuperPoint. 

\textbf{Baselines.} The baselines comprise of simple matchers such as MNN and NN-RT~\cite{sift}. Besides, filtering-based methods including OANet~\cite{oanet}, AdaLAM~\cite{adalam}, CLNet~\cite{clnet} and LMCNet~\cite{lmcnet} are also included. The final part is transformer-based matchers such as SuperGlue~\cite{superglue}, SGMNet~\cite{sgmnet}, and ClusterGNN~\cite{clustergnn}. As it's difficult to reproduce the results of SuperGlue from custom training (official training code is not released), we follow SGMNet and show results of original SuperGlue (SuperGlue*) and the model trained by SGMNet (SuperGlue).

\textbf{Comparison with filtering-based methods.} Table~\ref{tab:yfcc} shows our IMP and EIMP give higher accuracy than previous filtering-based approaches such as OANet~\cite{oanet} and LMCNet~\cite{lmcnet} for both RootSIFT~\cite{sift,rootsift2012} and SuperPoint~\cite{superpoint} keypoints. Because these methods rely purely on the geometric information to filter potentially wrong correspondences, their performance is influenced by the quality of initial matches. In contrast, we use both the geometric information and descriptors for matching, which are able to give more accurate matches, resulting in more precise poses.

\textbf{Comparison with matchers.} Augmented with spatial information, SuperGlue~\cite{superglue} and its variants~\cite{sgmnet,clustergnn} outperform MNN and NN-RT obviously. Although SGMNet~\cite{sgmnet} and ClusterGNN~\cite{clustergnn} work faster, they give worse accuracy than SuperGlue*. With embedded geometric information, our IMP outperforms SuperGlue*. By discarding outliers adaptively, our EIMP even gives slightly better results than SuperGlue*. Compared with IMP, our EIMP loses about 5\% matches and gains over 2\% more inliers.

Table~\ref{tab:scannet} shows results on the Scannet dataset~\cite{scannet}. Our IMP and EIMP also give higher accuracy than filtering-based approaches and matchers on RootSIFT keypoints. When using SuperPoint, our IMP gives slightly better performance than SuperGlue* and SGMNet, which have close performance to our EIMP. LMCNet~\cite{lmcnet} reports the best accuracy at error thresholds of $10^\circ$ and $20^\circ$ with SuperPoint because LMCNet uses SuperGlue* to provide initial matches and is further trained on the indoor dataset~\cite{sun3d2013}.

\textbf{Qualitative comparison.} As shown in Fig.~\ref{fig:match_comp}, in the iteration process, both IMP and EIMP produce more inliers and more accurate poses progressively. In addition, EIMP dynamically discards useless keypoints after each iteration to redundant computation. We also show the results of SuperGlue*~\cite{superglue} and SGMNet~\cite{sgmnet}. Due to large viewpoint changes, SGMNet gives much fewer inliers and has larger rotation and translation errors compared to SuperGlue* and our models. SuperGlue* yields more inliers than IMP and EIMP, but has larger errors because we embed geometric information implicitly into IMP and EIMP, enabling them to predict geometry-aware matches.
 
\begin{figure*}[t!]
 	\centering
 	\includegraphics[width=.99\linewidth]{images/match_comp_iterative}
 	\caption{\textbf{Qualitative comparison.} We visualize the iterative process (left$\rightarrow$right) of IMP (top) and EIMP (bottom). We also report the number inliers/matches and rotation/translation errors (bottom) and the number of preserved keypoints in two sets (top) at each iteration. \textcolor{green}{Inliers} between two images are visualized. More results and analysis are provided in the supplementary material.}
 	\label{fig:match_comp}
\end{figure*}

%\input{figs_tables/table_fm_bench}
%\input{figs_tables/table_fm_bench_usac}
\input{figs_tables/table_scannet_usac}


\subsection{Visual localization}
\label{sec:localization}

\textbf{Dataset and metrics.} We additionally test our method on large-scale localization task at Aachen Day-Night (v1.0 and v1.1) datasets~\cite{aachen,aachenv112021}. Aachen v1.0 dataset comprises of 4,328 reference and 922 query (824 day, 98 night) images. Aachen v1.1 extends v1.0 by adding additional 2,369 reference and 93 night query images. We use HLoc~\cite{hloc2019} for mapping and localization and report the accuracy at error thresholds of $0.25m/2^\circ$, $0.5m/5^\circ$, and $5m/10^\circ$.

\textbf{Baselines.} As most filtering-based methods~\cite{clnet, lmcnet, adalam} don't report results on the large-scale localization task, we only provide the results of OANet~\cite{oanet} (results are quoted from~\cite{sgmnet}). In addition, we mainly compare our method with prior SOTA transformer-based matchers including SuperGlue~\cite{superglue}, SGM~\cite{sgmnet}, and ClusterGNN~\cite{clustergnn}. As localization task requires only correspondences for mapping and localization, we only output the final matches and do not conduct pose estimation in the iterative process.

\textbf{Result analysis.} OANet~\cite{oanet} gives close accuracy to MNN at error thresholds of $0.25m, 2^\circ$ and $0.5m, 5^\circ$, but much better performance at error threshold of $5m, 10^\circ$, because test images with larger viewpoint changes are more sensitive to outliers which can be partially filtered by OANet. Our IMP obtains similar performance to SuperGlue*~\cite{superglue} and outperforms SGMNet~\cite{sgmnet} and ClusterGNN~\cite{clustergnn} especially for night images.

EIMP even slightly outperforms IMP and SuperGlue*. That is because in the long-term large-scale localization task, query and reference images usually have larger viewpoint and illumination changes, resulting in more keypoints without true matches. EIMP adaptively discards these keypoints and thus improves the accuracy. Similar results can also be observed in Fig.~\ref{fig:match_comp} where EIMP also boots the relative pose estimation at the first and second iterations.

\input{figs_tables/table_aachen}

\subsection{Running time}
\label{sec:running_time}

\begin{figure}[t]
	%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\centering
	\begin{subfigure}{.22\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/running_iteration}
		\caption{}
		\label{fig:num_iteration}
	\end{subfigure}\quad
	\begin{subfigure}{.22\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/running_time}
		\caption{}
		\label{fig:total_time}
	\end{subfigure}
	\caption{\textbf{Running time analysis.} We show (a) the number of iterations required for each pair YFCC100m dataset~\cite{yfcc100m} and (b) the mean running time of 1k pairs on RTX 3090.}
	\label{fig:running_time}
\end{figure}
 
As the source code of ClusterGNN~\cite{clustergnn} is not released, we mainly compare our method with SuperGlue*~\cite{superglue} and SGMNet~\cite{sgmnet}. The total time for each method is the summary of the time used at each iteration. IMP reduces the time by reducing the number of iterations and EIMP further decreases the time of each iteration.
 
Fig.~\ref{fig:num_iteration} shows the number of iterations for relative pose estimation on YFCC100m dataset~\cite{yfcc100m}. SuperGlue*~\cite{superglue} and SGMNet~\cite{sgmnet} adopt a fixed number of layers and only give matches at the last layer, so they don't report any results before the last iteration. In contrast, in our iterative framework, IMP needs only 4 iterations for 30\% cases and 5 iterations for 55\% cases, avoiding extra computation. EIMP performs slightly worse than IMP because of matches loss, as discussed in Sec.~\ref{sec:dyn_attn}. Fig.~\ref{fig:total_time} shows the running time of SuperGlue*, SGMNet, IMP and EIMP. When using 1k and 2k keypoints, IMP and EIMP run slower than SuperGlue* because the shared attention introduces additional cost. However, when using more than 3k keypoints, IMP runs faster because it uses fewer number of iterations (10) for sinkhorm optimization~\cite{sinkhorn1967,sinkhorn2013}. Benefiting from adaptive pooling strategy, EIMP works even faster than SGMNet when using keypoints less than 6k but gives better accuracy, as demonstrated in Table~\ref{tab:yfcc}.

\subsection{Ablation study}
\label{sec:ablation}
We conduct a full ablation study on YFCC100m dataset~\cite{yfcc100m} with SuperPoint~\cite{superpoint} to verify all components in our model including the shared attention (S), geometric loss (G), pose-aware iteration (P), adaptive pooling (A), and adaptive pooling with pose uncertainty (U).

Table~\ref{tab:ablation_yfcc} shows that shared attention (S) improves both the pose and matching accuracy. Geometric loss (G) and pose-aware iteration (P) also enhances the performance of IMP and EIMP. Comparisons between IMP-SG and EIMP-SGA indicate that our adaptive pooling reduces 5\% matches and increases 1\% inliers. The pose uncertainty (U) further increases the number of matches and enhances the pose estimation by dynamically adjusting the pooling ratio. With ratio-based pooling, EIMP-S, gives promising pose accuracy while loses over 10\% matches than our adaptive pooling, EIMP-SA, whcih effectively mitigates this problem.

\input{figs_tables/table_ablation_yfcc100m}
%Table~\ref{tab:ablation_aachen} shows the efficacy of geometric loss to the visual localization task. With geometric loss, both the full and efficient models give higher accuracy, while the improvement is relatively small compared to the relative pose estimation in Table~\ref{tab:ablation_yfcc}. 
